Precision measurements of the top quark mass from the Tevatron in the pre-LHC era

The top quark is the heaviest of the six quarks of the Standard Model. Precise knowledge of its mass is important for imposing constraints on a number of physics processes, including interactions of the as yet unobserved Higgs boson. The Higgs boson is the only missing particle of the Standard Model, central to the electroweak symmetry breaking mechanism and generation of particle masses. In this Review, experimental measurements of the top quark mass accomplished at the Tevatron, a proton-antiproton collider located at the Fermi National Accelerator Laboratory, are described. Topologies of top quark events and methods used to separate signal events from background sources are discussed. Data analysis techniques used to extract information about the top mass value are reviewed. The combination of several most precise measurements performed with the two Tevatron particle detectors, CDF and \D0, yields a value of $\Mt = 173.2 \pm 0.9$ GeV/$c^2$.

==> Makefile <==
TEXFILES = combination.tex conclusions.tex definitions.tex \
           identifying_top.tex introduction.tex measurements_allhad.tex \
           measurements_ljets.tex measurements_other.tex \
           measurement_techniques.tex monte_carlo_modeling.tex \
           production_and_decay.tex references.tex systematics.tex \
           measurements_dilep.tex tev_measurements.tex \
           mass_from_sigma.tex measurements_metjets.tex

FIGURES = Plots/2009_ttbarxs_vsmass-1.eps Plots/cdf_btag_eff_ttbar.eps \
          Plots/cdfii_3d_p1.eps Plots/cdfii_track_z.eps Plots/d0_btag_eff.eps \
          Plots/d0_detector.eps Plots/d0_tracker.eps  \
          Plots/btagging_cartoon.eps \
          Plots/jet_sys_cdf.eps Plots/mt_mw_2009.eps \
          Plots/d0_jes_error_vs_et_cone5_gamjet_eta1.0.eps \
          Plots/quigg_tmass_history.eps \
          Plots/sigma-vs-mhiggs.eps Plots/tev_sigma_vs_mhiggs.eps \
          Plots/top_decays_square.eps Plots/top_pie_chart.eps \
          Plots/top_prod_diagrams.eps Plots/top_w_higgs_diagrams.eps \
          Plots/ttbar_sig_l+jet_njets_method2.eps Plots/TevSum10combo.eps \
          Plots/cdf_mistag_eff_ttbar.eps Plots/d0_njeq3_btagonlyT11AF03b.eps \
          Plots/d0_njgt3_btagonlyT11AF03a.eps\
          Plots/d0_tf.eps Plots/mlnu.eps \
          Plots/d0_dilepton_likelihood.eps Plots/cdf_ljets_likelihood.eps \
          Plots/d0_sig_mass_T11FF01.eps \
          Plots/final_nn_discrim_gen6_masses.eps Plots/mt_templates.eps \
          Plots/d0_dlb.eps Plots/d0_dilep_nuwt.eps Plots/cdf_chisq_distro.eps \
          Plots/mt2_tagged.eps Plots/mtnwa_tagged.eps Plots/lxy_dist_comp.eps \
          Plots/htop_mt_ttop25.eps Plots/htop_mT2_ttop25.eps Plots/dsdtpt.eps \
          Plots/d0_ljets_result.eps Plots/LepPt_dist_comp.eps \
          Plots/fig2fromd0mdelta_a.eps Plots/fig2fromd0mdelta_b.eps \
          Plots/met_comparison_56invfb.eps Plots/cdf-compare.eps
          
all: top_mass_paper.pdf top_mass_paper_2c.pdf 
# all: top_mass_paper.pdf
# all: top_mass_paper_2c.pdf

top_mass_paper.dvi: top_mass_paper.tex $(TEXFILES) $(FIGURES)
	latex top_mass_paper.tex
	latex top_mass_paper.tex

top_mass_paper.ps: top_mass_paper.dvi
	dvips -t a4 -o $@ $<

top_mass_paper.pdf: top_mass_paper.ps
	ps2pdf -sPAPERSIZE=a4 top_mass_paper.ps

top_mass_paper_2c.dvi: top_mass_paper_2c.tex $(TEXFILES) $(FIGURES)
	latex top_mass_paper_2c.tex
	latex top_mass_paper_2c.tex

top_mass_paper_2c.ps: top_mass_paper_2c.dvi
	dvips -t a4 -o $@ $<

top_mass_paper_2c.pdf: top_mass_paper_2c.ps
	ps2pdf -sPAPERSIZE=a4 top_mass_paper_2c.ps

clean:
	rm -f *~ *.log *.aux *.dvi *.bak


==> definitions_rev.tex <==
% definitions
\def \Etmiss {{\not}{E_T}}
\def \mW {$m_W$}
%\def \mt {$m_t$}
\def \mH {$m_H$}
\def \lum {\cal L}
\def \gevocs {$GeV/c^2$ }
\def \gevoc {$GeV/c$ }
\def \D0  {D\O} 
\def \mt {\ensuremath m_t}
\def \into {\rightarrow}

% another set
\newcommand{\met}{\rm\,/\!\!\!\!E_{T}}
\newcommand{\ppbar}{p\bar{p}}
\newcommand{\ttbar}{t\bar{t}}
\newcommand{\bbbar}{b\bar{b}}
\newcommand{\ccbar}{c\bar{c}}
\newcommand{\ppbb} { \ppbar \rightarrow  \bbbar }
\newcommand{\tbar}{\bar{t}}
\newcommand{\deltar}{\sqrt{\Delta \eta ^{2}+ \Delta \phi ^{2}}}

%
%---------- UNITS, SYMBOLS
%
\newcommand{\nb}{ {\rm nb} }
\newcommand{\pb}{ {\rm pb} }
\newcommand{\imb}{ \mu {\rm b}^{-1} }
\newcommand{\inb}{ {\rm nb}^{-1} }
\newcommand{\ipb}{ {\rm pb}^{-1} }
\newcommand{\ifb}{ {\rm fb}^{-1} }
\newcommand{\degs}{\mbox{$^{\circ}$}}
%\newcommand{\gsim}{\mbox{\small$\stackrel{>}{\sim}$\normalsize}}
%\newcommand{\lsim}{\mbox{\small$\stackrel{<}{\sim}$\normalsize}}

%
%---------- Journal names
%
%\newcommand{\prl}[1]{Phys. Rev. Lett {\bf #1}}
%\newcommand{\prl}{\rm Phys. Rev. Lett}
%\newcommand{\prev}{\it {Phys. Rev.}}
%\newcommand{\prd}{\it Phys. Rev. D} 
\newcommand{\zs}{\it {Z. Phys. }}
\newcommand{\ncim}{\protect{\it Nuovo Cim.} }
\newcommand{\plet}{\protect{\it Phys. Lett. }}
\newcommand{\prep}{\protec{\it Phys. Rep. }}
\newcommand{\rmp}{\protect{\it Rev. Mod. Phys. }}
\newcommand{\nphy}{\protect{\it Nucl. Phys. }}
%\newcommand{\nim}{\it {Nucl. Instrumen. Meth.}}

\def \prl {\protect {\it {Phys. Rev. Lett}}}
\def \prev {\protect {\it {Phys. Rev.}}}
\def \prd {\protect {\it {Phys. Rev. D}}}
\def \nim {\protect {\it{Nucl. Instrumen. Meth }}}
\def \rpp {\protect {\it{Rep. Prog. Phys }}}
\def \plep {\protect {\it{Phys. Lett. }}}
\def \nphy {\protect {\it {Nucl. Phys. }}}

% abbreviations for IOPP journals
%
\newcommand{\CQG}{{\it Class. Quantum Grav.} }
\newcommand{\CTM}{{\it Combust. Theory Modelling\/} }
\newcommand{\DSE}{{\it Distrib. Syst. Engng.\/} }
\newcommand{\EJP}{{\it Eur. J. Phys.} } 
\newcommand{\JNE}{{\it J. Neural Eng.} } %added 30/11/2004 GMD
\newcommand{\PB}{{\it Phys. Biol.} } %added 30/11/2004 GMD
\newcommand{\SMS}{{\it Smart Mater. Struct.} } %added 30/11/2004 GMD
\newcommand{\HPP}{{\it High Perform. Polym.} }              % added 4/5/93
\newcommand{\IP}{{\it Inverse Problems\/} }
\newcommand{\JHM}{{\it J. Hard Mater.} }                    % added 4/5/93
\newcommand{\JO}{{\it J. Opt.} }
\newcommand{\JOA}{{\it J. Opt. A: Pure Appl. Opt.} }
\newcommand{\JOB}{{\it J. Opt. B: Quantum Semiclass. Opt.} }
\newcommand{\JPA}{{\it J. Phys. A: Math. Gen.} }
\newcommand{\JPB}{{\it J. Phys. B: At. Mol. Phys.} }      %1968-87
\newcommand{\jpb}{{\it J. Phys. B: At. Mol. Opt. Phys.} } %1988 and onwards
\newcommand{\JPC}{{\it J. Phys. C: Solid State Phys.} }   %1968--1988
\newcommand{\JPCM}{{\it J. Phys.: Condens. Matter\/} }    %1989 and onwards
\newcommand{\JPD}{{\it J. Phys. D: Appl. Phys.} }
\newcommand{\JPE}{{\it J. Phys. E: Sci. Instrum.} }
\newcommand{\JPF}{{\it J. Phys. F: Met. Phys.} }
\newcommand{\JPG}{{\it J. Phys. G: Nucl. Phys.} }         %1975--1988
\newcommand{\jpg}{{\it J. Phys. G: Nucl. Part. Phys.} }   %1989 and onwards
\newcommand{\JMM}{{\it J. Micromech. Microeng.\/} }
\newcommand{\MSMSE}{{\it Modelling Simulation Mater. Sci. Eng.} }
\newcommand{\MST}{{\it Meas. Sci. Technol.} }                 %1990 and onwards
\newcommand{\NET}{{\it Network: Comput. Neural Syst.} }
\newcommand{\NJP}{{\it New J. Phys.} }
\newcommand{\NL}{{\it Nonlinearity\/} }
\newcommand{\NT}{{\it Nanotechnology} }
\newcommand{\PAO}{{\it Pure Appl. Optics\/} }
\newcommand{\PM}{{\it Physiol. Meas.} }                        % added 4/5/93
\newcommand{\PMB}{{\it Phys. Med. Biol.} }
\newcommand{\PPCF}{{\it Plasma Phys. Control. Fusion\/} }      % added 4/5/93
\newcommand{\PSST}{{\it Plasma Sources Sci. Technol.} }
\newcommand{\PUS}{{\it Public Understand. Sci.} }
\newcommand{\QO}{{\it Quantum Opt.} }
\newcommand{\QSO}{{\em Quantum Semiclass. Opt.} }
\newcommand{\RPP}{{\it Rep. Prog. Phys.} }
\newcommand{\SLC}{{\it Sov. Lightwave Commun.} }               % added 4/5/93 
\newcommand{\SST}{{\it Semicond. Sci. Technol.} }
\newcommand{\SUST}{{\it Supercond. Sci. Technol.} }
\newcommand{\WRM}{{\it Waves Random Media\/} }
%
% Other commonly quoted journals
%
\newcommand{\AC}{{\it Acta Crystallogr.} }
\newcommand{\AM}{{\it Acta Metall.} }
\newcommand{\AP}{{\it Ann. Phys., Lpz.} }
\newcommand{\APNY}{{\it Ann. Phys., NY\/} }
\newcommand{\APP}{{\it Ann. Phys., Paris\/} }
\newcommand{\CJP}{{\it Can. J. Phys.} }
\newcommand{\JAP}{{\it J. Appl. Phys.} }
\newcommand{\JCP}{{\it J. Chem. Phys.} }
\newcommand{\JJAP}{{\it Japan. J. Appl. Phys.} }
\newcommand{\JP}{{\it J. Physique\/} }
\newcommand{\JPhCh}{{\it J. Phys. Chem.} }
\newcommand{\JMMM}{{\it J. Magn. Magn. Mater.} }
\newcommand{\JMP}{{\it J. Math. Phys.} }
\newcommand{\JOSA}{{\it J. Opt. Soc. Am.} }
\newcommand{\JPSJ}{{\it J. Phys. Soc. Japan\/} }
\newcommand{\JQSRT}{{\it J. Quant. Spectrosc. Radiat. Transfer\/} }
\newcommand{\NC}{{\it Nuovo Cimento\/} }
\newcommand{\NIM}{{\it Nucl. Instrum. Methods\/} }
\newcommand{\NP}{{\it Nucl. Phys.} }
\newcommand{\PL}{{\it Phys. Lett.} }
\newcommand{\PR}{{\it Phys. Rev.} }
\newcommand{\PRL}{{\it Phys. Rev. Lett.} }
\newcommand{\PRS}{{\it Proc. R. Soc.} }
\newcommand{\PS}{{\it Phys. Scr.} }
\newcommand{\PSS}{{\it Phys. Status Solidi\/} }
\newcommand{\PTRS}{{\it Phil. Trans. R. Soc.} }
\newcommand{\RMP}{{\it Rev. Mod. Phys.} }
\newcommand{\RSI}{{\it Rev. Sci. Instrum.} }
\newcommand{\SSC}{{\it Solid State Commun.} }
\newcommand{\ZP}{{\it Z. Phys.} }
%
\pagestyle{headings}



% \rppbib command arguments for standard journal references
%
% 1. label (must be unique)
% 2. authors
% 3. year of publication
% 4. journal
% 5. volume number
% 6. pages (including end page)
%
\newcommand{\rppbib}[6]{
  \bibitem{#1}
  #2 #3 #4 {\bf #5} #6}

\newcommand{\sub}[1]{\ensuremath{_{\mbox{\scriptsize \,#1}}}}
\newcommand{\supers}[1]{\ensuremath{^{\mbox{\scriptsize #1}}}}

\def\Mt {{\it M}\sub{t}}
\def\etal {\protect {\it et al}}

\newenvironment{mylist} {
    \begin{list} {---} {
    }
} {\end{list}}

